Towards Identifying Human Actions, Intent, and Severity of APT Attacks Applying Deception Techniques -- An Experiment

Attacks by Advanced Persistent Threats (APTs) have been shown to be difficult to detect using traditional signature- and anomaly-based intrusion detection approaches. Deception techniques such as decoy objects, often called honey items, may be deployed for intrusion detection and attack analysis, providing an alternative to detect APT behaviours. This work explores the use of honey items to classify intrusion interactions, differentiating automated attacks from those which need some human reasoning and interaction towards APT detection. Multiple decoy items are deployed on honeypots in a virtual honey network, some as breadcrumbs to detect indications of a structured manual attack. Monitoring functionality was created around Elastic Stack with a Kibana dashboard created to display interactions with various honey items. APT type manual intrusions are simulated by an experienced pentesting practitioner carrying out simulated attacks. Interactions with honey items are evaluated in order to determine their suitability for discriminating between automated tools and direct human intervention. The results show that it is possible to differentiate automatic attacks from manual structured attacks; from the nature of the interactions with the honey items. The use of honey items found in the honeypot, such as in later parts of a structured attack, have been shown to be successful in classification of manual attacks, as well as towards providing an indication of severity of the attacks

==> sections/background.tex <==
\section{Background}
\label{sec:background}



\todo{
\begin{itemize}
    \item don't worry too much about defining APTs and the attack environment, the high level work should largely be left to the introduction
    \item what work has been done in identifying APTs?
    \item relevant AI/ML/heuristics
    \item work in honey nets / honey tokens
    \item work in detecting humans rather than automated tools/bots
    \item should be around 1-1.5 pages
\end{itemize}
}

==> sections/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

\todo{
\begin{itemize}
    \item brief summary of what was achieved, recap the contributions
    \item take-away and implications
    \item future work
    \item ideally should be relatively short, half a page
\end{itemize}
}

==> sections/findings.tex <==
\section{Findings}
\label{sec:findings}


\todo{
\begin{itemize}
    \item findings with relevant tables
    \item make sure to have clear evidence for each contribution/research question
    \item keep a clean narrative
    \item figures for crucial components
    \item this section should do most of the work in the paper. 2-3 pages
\end{itemize}
}

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

\todo{
\begin{itemize}
    \item brief context
    \item roughly of the shape:
        \begin{itemize}
            \item general note about digital landscape
            \item crime, hacking APTs
            \item detecting APTs challenging
            \item current stuff not great, gap
            \item bit about detecting human interaction rather than just automated scans/tools
            \item brief description of general solution
        \end{itemize}
    \item then have either a list of research questions or contributions.
    \item shouldn't be much more than page total. ideally would fit on the first page, though don't worry it not.
    \end{itemize}
RICH: 
Contribution could be building on previous work in the field around APT/structured attack detection and analysis, focusing on human vs automated attack detection and tracking using honey network and honey tokens. 
Successfully shown a honey network and honey tokens can be used to detect and categorise human and automated type attacks as part of structured attack process?
}

==> sections/method.tex <==
\section{Methodology}
\label{sec:methodology}


\todo{
\begin{itemize}
    \item focused methodology with specifics on setup, and measurements taken
    \item what was the network setup like?
    \item what assumptions were made?
    \item how are the tokens used justified?
    \item what was the human test setup/condition?
\end{itemize}
RICH:
We want to have a method which builds on/draws from other research, from the related work/lit review. 
A focus on the automated vs human interaction activities -  your table showing these is a great start on this. }


